Simple and Effective Unsupervised Speech Synthesis

We introduce the first unsupervised speech synthesis system based on a simple, yet effective recipe. The framework leverages recent work in unsupervised speech recognition as well as existing neural-based speech synthesis. Using only unlabeled speech audio and unlabeled text as well as a lexicon, our method enables speech synthesis without the need for a human-labeled corpus. Experiments demonstrate the unsupervised system can synthesize speech similar to a supervised counterpart in terms of naturalness and intelligibility measured by human evaluation.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> sections/setup.full.tex <==
\section{Experimental Setup}
\label{sec:setup}

\noindent\subsection{Dataset}\label{subsec:dataset}

\noindent\textbf{Audio.}
Two scenarios are considered:
\begin{itemize}
    \item \textbf{Single speaker}: {LJSpeech}~\cite{ljspeech17} contains 13,100 utterances ($\approx$24 hours) of read speech from a single female speaker, sampled at 22khz. 
    Following prior works on weakly-supervised TTS~\cite{ren2019almost,liu2020towards}, 300 utterances are randomly selected for both validation and test set, leaving 12500 utterances for training.
    \item \textbf{Multi-speaker}: {LibriTTS}~\cite{zen2019libritts} is a subset derived from LibriSpeech~\cite{panayotov2015librispeech} containing over 500 hours of speech collected from 2456 speakers, with sampling rate at 24khz. 
    We used the \texttt{\footnotesize{train-clean}} subsets combining roughly 250 hours for training.
    Since unseen speaker modeling is not our focus, we followed the original work~\cite{zen2019libritts} and randomly selected 6 speakers (three males and three females with IDs {\footnotesize\texttt{8699, 4535, 6209, 6701, 3922, 3638}}) from training split and use text from \texttt{\footnotesize{test-clean}} for testing.
\end{itemize}

% \noindent\textbf{Audio.} LJSpeech~\cite{ljspeech17} is used as the unpaired audio source. It contains 13,100 utterances ($\approx$24 hours) of read speech from a single female speaker. Following prior work on weakly-supervised TTS~\cite{ren2019almost,liu2020towards}, 300 utterances are randomly selected for both validation and testing, leaving 12,500 utterances for training.
\noindent For unsupervised ASR, the audio is downsampled to 16khz to extract speech representations from wav2vec 2.0~\cite{baevski2020wav} to serve as the input.
For TTS, target Mel-spectrograms are extracted from the silence-removed audio with 80 Mel filter banks.

\vspace{4pt}

\noindent\textbf{Text.} The official text corpus provided by LibriSpeech~\cite{panayotov2015librispeech} is used as the unpaired text source. Transcriptions of utterance from LJspeech/LibriTTS are excluded\footnote{ \scriptsize\url{https://github.com/flashlight/wav2letter/blob/main/recipes/sota/2019/raw_lm_corpus/README.md}} to ensure there is no exact match between text and audio data.

\vspace{4pt}

\noindent\textbf{Lexicon.}
A word-to-phone mapping is obtained through an off-the-shelf phonemeizer~\cite{g2pE2019}.
To phonemize the text source, all punctuation marks are discarded and the difference between variants of the same phone is ignored.
This results in a phoneme inventory with a size of 39 used for both the ASR and the TTS.

\noindent\subsection{Unsupervised ASR model}
\label{setup:asr}
\noindent\textbf{Training.} Wav2vec-U 2.0~\cite{liu2022towards} is used for pseudo-labeling unpaired speech.
The recognizer is a 3-layer network taking 1024 dimensional speech representation as input.
Input feature is first normalized and rescaled with batch normalization, followed by a linear projection, and a convolution neural network taking 9 frames at a time with a stride of 3 to predict the underlying phone.
To output the sequence of phone prediction, consecutive predictions sharing the same most likely phone will be merged into a single prediction by random selection.
The recognizer is trained with adversarial learning against a discriminator composed of a 2-layer convolutional neural network with a receptive field of size 9.
The discriminator is trained to distinguish between the recognizer output sequence predictions from the one-hot vector sequences representing phone sequences from the unpaired text.
Conversely, the recognizer is trained to mislead the discriminator into classifying its output as real phone sequence.
We use the fairseq~\cite{ott2019fairseq} implementation for training with default hyper-parameter\footnote{\scriptsize\url{https://github.com/pytorch/fairseq/tree/main/examples/wav2vec/unsupervised}}.

\vspace{4pt}

\noindent\textbf{Decoding.} To transcribe the unpaired audio after wav2vec-U 2.0 training, each utterance is decoded by the recognizer together with a phoneme-to-phoneme WFST~\cite{mohri2002weighted} (including a phone-based 6-gram language model trained from the lexicon-phomenized text corpora).
Beam search with beam size 15 is used for decoding with hyper-parameters selected with an unsupervised metric~\cite{baevski2021unsupervised}.
As a reference, decoding the test set with this unsupervised ASR results in 6.97\%/7.78\% phone error rate on LJSpeech/LibriTTS respectively.



\noindent\subsection{TTS model}
\label{setup:tts}
\noindent\textbf{Text-to-Speech}
Transformer-TTS~\cite{li2019neural}, a sequence-to-sequence encoder-decoder model, is selected as the phone-to-mel-spectrogram model in our framework.
Transformer-TTS consists of an encoder, an auto-regressive decoder, a pre-net, and a post-net. 
The encoder and decoder have 6 layers of transformer blocks.
The training objective is to minimize the L2 reconstruction error between the model output and the targeted Mel-spectrogram corresponded to the input text.
We used ESPNet-TTS~\cite{hayashi2020espnet} for model training based on its default configurations\footnote{\scriptsize\url{https://github.com/espnet/espnet/tree/master/egs2/}}.
On LJspeech, we found that it is necessary to enforce guided attention loss~\cite{tachibana2018efficiently} in \textit{all} 48 decoder attention heads, while the same does not hold true for LibriTTS.
% Increasing the guided attention weights while only enforcing it on parts of the attention heads does not improve synthesis quality.
We tripled the number of training epochs from 200 to 600 for LJspeech, while keeping the training epochs to 1000 for LibriTTS. 
Furthermore, we found that Tacotron2~\cite{shen2018natural} has worse synthesis quality and Fastspeech2~\cite{ren2020fastspeech} has issues synthesizing longer utterances. 
We hypothesized all these difficulties arose due to the use of a reduced phone sets (see Lexicon in Section~\ref{subsec:dataset}), which makes the text to Mel-spectrogram mapping much more difficult in the absence of pronunciation.
Model selection is based on validation loss, and the best 5 checkpoints are decoded and averaged. 

\vspace{2pt}
\noindent\textbf{Speaker and Style Modeling}
On LibriTTS, speaker embeddings from a pre-trained speaker verification model~\cite{jia2018transfer} and Global Style Tokens (GST)~\cite{wang2018style} are trained in conjunction with Transformer-TTS for multi-speaker and style modelings. 
Given the large number of training speakers, we opted for the latest speaker verification model ECAPA-TDNN~\cite{desplanques2020ecapa}, as TTS speaker modeling is correlated to its speaker encoder~\cite{cooper2020zero,xue2022ecapa}.
ECAPA-TDNN was taken from SpeechBrain~\cite{ravanelli2021speechbrain} and pre-trained on Voxceleb 1 and 2 with a 0.69\% EER\footnote{https://huggingface.co/speechbrain/spkrec-ecapa-voxceleb}. 
To further improve speaker modeling, we took the multi-speaker Transformer-TTS and further perform target speaker finetuning for each target speaker. 
Only 10 epoches of finetuning is enough, while significantly improving the synthesis quality.

\vspace{2pt}

\noindent\textbf{Vocoder} 
A separate vocoder pre-trained on the same corpus converts the synthesized mel-spectrograms into waveforms. 
On LJspeech, we chose Parallel WaveGAN~\cite{yamamoto2020parallel} that was trained for 3M iterations.
On LibriTTS, HiFi-GAN~\cite{kong2020hifi} produces the clearest speech compared to MelGAN~\cite{kumar2019melgan} and Parllalel WaveGAN. 
Subsequently, we adopted HiFi-GAN for the remaining experiments. 
The three vocoders are publicly available\footnote{\scriptsize\url{https://github.com/kan-bayashi/ParallelWaveGAN}}. 

%\noindent\textbf{Failed Models}
% --> only for LibriTTS

\noindent\subsection{Evaluation}
To evaluate the proposed unsupervised TTS method, we compare the speech quality of the following settings:
\begin{itemize}
    \item \textbf{{Unsupervised} ({\tt Unsup})}: synthetic speech from the unsupervised TTS model.
    \item \textbf{{Supervised} ({\tt Sup})}: synthetic speech from supervised topline -- the same TTS model trained with ground truth transcription instead of machine annotation.
    \item \textbf{{Natural} ({\tt Nat})}:  speech  from the dataset.
\end{itemize}

\noindent Three subjective and objective measures are conducted:
\begin{itemize}
    \item \textbf{Mean Opinion Score (MOS)}~: quantifies subjective naturalness, where workers are asked to rate each utterance on a 5-point scale (with 1-point increment).
    We ran 150 HITs (crowdsourced tasks) for LJspeech and 200 HITs for LibriTTS to compare the synthesis quality between {\tt Unsup}, {\tt Sup} and {\tt Nat}. 
    100 unique utterances respectively from LJspeech and LibriTTS test sets are selected randomly and designated as the MOS test sets.  
    For a HIT on LJspeech, 10 utterances from its MOS test set are chosen for {\tt Nat} and synthesized for {\tt Unsup} and {\tt Sup}, for a total of 30 utterances.
    For a HIT on LibriTTS, 3 utterances from its MOS test set are chosen for {\tt Nat} and synthesized for {\tt Unsup} and {\tt Sup} for each one of the 6 target speakers, for a total of 39 utterances.
    
    % The order presented to the workers is random.
    
    \item \textbf{Word Error Rate (WER)}~: quantifies intelligibility.
    The LJspeech test set (300 synthetic utterances) is fed into Google's ASR API\footnote{\scriptsize\url{https://pypi.org/project/SpeechRecognition/}}
    and we measure the word error rate of the result with respect to the input ground truth.
    
    \item \textbf{Pairwise Opinion Score}~: quantifies subjective pair-wise naturalness and intelligibility (also known as A/B test), where workers are asked to select the more natural or intelligible synthesized utterances between {\tt Unsup} and {\tt Sup}. 
    We ran it for 1000 HITs, and in each HIT, a random utterance is drawn from the MOS test set, synthesized, and presented to the workers.  
    
\end{itemize}

